Mirror-Aware Neural Humans

Human motion capture either requires multi-camera systems or is unreliable when using single-view input due to depth ambiguities. Meanwhile, mirrors are readily available in urban environments and form an affordable alternative by recording two views with only a single camera. However, the mirror setting poses the additional challenge of handling occlusions of real and mirror image. Going beyond existing mirror approaches for 3D human pose estimation, we utilize mirrors for learning a complete body model, including shape and dense appearance. Our main contributions are extending articulated neural radiance fields to include a notion of a mirror, making it sample-efficient over potential occlusion regions. Together, our contributions realize a consumer-level 3D motion capture system that starts from off-the-shelf 2D poses by automatically calibrating the camera, estimating mirror orientation, and subsequently lifting 2D keypoint detections to 3D skeleton pose that is used to condition the mirror-aware NeRF. We empirically demonstrate the benefit of learning a body model and accounting for occlusion in challenging mirror scenes.

==> figures/loc_smooth_scale.tex <==
\begin{figure} [!ht]%
% \begin{center}
\includegraphics[width=0.49\linewidth,trim={0.0 0.0 2.5 0.0},clip]{images/orient_smooth_scale_cam3_recreated2.png}
\includegraphics[width=0.49\linewidth,trim={0.0 0.0 2.5 0.0},clip]{images/loc_smooth_scale_cam3_recreated2.png}
% \end{center}
  \caption{Ablation study on smoothness terms, all values in P-MPJPE. \textbf{Left:} Effect of the angular smoothness weight \textbf{Right:} Effect of the positional smoothness weight.  
  }
\label{fig:ablation-location} 
\end{figure}%

==> figures/mirror_retarget.tex <==
\begin{figure}[!ht]%
% \begin{center}
\includegraphics[width=1.0\linewidth,trim={0.0cm 0 0cm 0},clip]{images/Ti_mirror_retarget.pdf}
% \end{center}
\dotcaption{Mirror Retargeting} {Given a source body (left), Mirror-Aware Neural Humans successfully simulate the mirror arrangement in an unseen setting (right).}
\label{fig:mirror_retarget}  
\end{figure}%

==> figures/novel_pose_synthesis.tex <==
\begin{figure}[ht]
    % \centering


\centering
\includegraphics[width=.2\textwidth]{pngs/raw_00001022_cropped.jpg}%\hfill
\includegraphics[width=.2\textwidth]{pngs/raw_00001022_side_view_cropped.png}%\hfill
\includegraphics[width=.2\textwidth]{pngs/raw_00001022_side_top_view_cropped.png}

\caption{default}
\label{fig:figure3}
    \caption{\textbf{Dynamic human motion rendering on the SURREAL dataset.} The 3D human pose and view are both unseen during training time. UNeRF-Conv preserves better finger structure  than the other architectures and achieves better results than the full capcity NeRF baseline when fully trained.}
    \label{fig:anerf}
\end{figure}

==> figures/pose_refinement.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth,trim={0cm 0 0cm 0cm},clip]{images/pose_refine7.pdf}
  \caption{\textbf{Qualitative results of pose refinement on \emph{MirrorHuman-eval} dataset~\cite{fang2017rmpe}} {Compared to SPIN~\cite{kolotouros2019spin} and A-NeRF~\cite{su2021nerf}, our Mirror A-NeRF} better aligns the skeleton model to the images.}
\label{fig:pose_refinement_visual} 
\end{figure}

==> figures/skel_3D_reprojection.tex <==
\begin{figure*}[t]%
\centering
% \begin{center}
\includegraphics[width=0.8\linewidth,trim={0.0cm 0 2.5cm 0},clip]{images/3D_reprojection.pdf}
% \end{center}
\dotcaption{Volumetric body model and 3D skeleton overlay} {Besides the ones provided in the main paper, we here show additional qualitative results on new actors and scenes. The skeleton overlay reveals how precise the fit is, even in unusual poses.}
\label{fig:skel_reprojection}  
\end{figure*}%

==> figures/step2_recon.tex <==
\begin{figure}[!b]%
\begin{center}
\includegraphics[width=1.0\linewidth,trim={0.0cm 0 0cm 0},clip]{images/step2_3D_recon.pdf}
\end{center}
\dotcaption{Mirror 3D reconstruction} {Our mirror approach successfully reconstructs challenging virtual poses in the mirror from the side and top view from scratch, including an extreme case of lying on the ground.}
\label{fig:virtual_pose}  
\end{figure}%

==> figures/supp_novel_views.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=1.0\linewidth,trim={0.0cm 0.0 0.0cm 0.0cm},clip]{images/supp_novel_views7.pdf}
  \caption{\textbf{Novel view synthesis results}. The learned reconstruction is a proper 3D model that can be rotated to novel views.}
\label{fig:supp_novel_views} 
\end{figure}

==> tables/bbox_iou_ratio.tex <==

\begin{table}[!ht]
\centering
  \resizebox{0.7\linewidth}{!}{%
\begin{tabular}{|l|cc|cc|}
\hline
$>$ IOU score &  \multicolumn{2}{c|}{No of Overlap Frames}   & \multicolumn{2}{c|}{Frame Ratio}  \\
\hline
 &  C6 & C7 & C6 & C7    \\
 \hline
5\%  & 402 & 652  & 0.25\% & 0.42\%  \\
7\%   & 322 & 569 & 0.20\% & 0.36\%  \\
\cellcolor{lightgray!25} 10\%  &  \cellcolor{lightgray!25} 229 & \cellcolor{lightgray!25}  450  & \cellcolor{lightgray!25} 0.14\% & \cellcolor{lightgray!25} 0.29\% \\
\cellcolor{gray!25} 20\%  &  \cellcolor{gray!25} 63 & \cellcolor{gray!25}  72 & \cellcolor{gray!25} \cellcolor{gray!25} 0.04\% & \cellcolor{gray!25} 0.05\%   \\
\hline
% \hline
% 5\% & 16.1\% & 32.2\% & 261 & 504    \\
% 7\%  & 13.1\% & 28.0\% & 212 & 438    \\
% \cellcolor{lightgray!25} 10\%  & \cellcolor{lightgray!25} 8.0\% & \cellcolor{lightgray!25} 20.2\% & \cellcolor{lightgray!25} 128 & \cellcolor{lightgray!25} 315    \\
% \cellcolor{gray!25} 20\%  & \cellcolor{gray!25} \cellcolor{gray!25} 2.4\% & \cellcolor{gray!25} 2.4\% &  \cellcolor{gray!25} 40 & \cellcolor{gray!25} 37    \\
% \hline
\end{tabular}}
\shortcaption{Number of candidate frames and ratio} {in cameras 6 and 7 automatically identified as overlapping cases based on their bounding box IOU score, thereby selecting the option with the highest confidence ($>$20\%). 
% \textcolor{red}{Please update Table values}.
}
\label{tab:box_iou}
\end{table}

